Fast, Accurate, and Simple Models for Tabular Data via Augmented Distillation

Automated machine learning (AutoML) can produce complex model ensembles by stacking, bagging, and boosting many individual models like trees, deep networks, and nearest neighbor estimators. While highly accurate, the resulting predictors are large, slow, and opaque as compared to their constituents. To improve the deployment of AutoML on tabular data, we propose FAST-DAD to distill arbitrarily complex ensemble predictors into individual models like boosted trees, random forests, and deep networks. At the heart of our approach is a data augmentation strategy based on Gibbs sampling from a self-attention pseudolikelihood estimator. Across 30 datasets spanning regression and binary/multiclass classification tasks, FAST-DAD distillation produces significantly better individual models than one obtains through standard training on the original data. Our individual distilled models are over 10x faster and more accurate than ensemble predictors produced by AutoML tools like H2O/AutoSklearn.

==> tables/openml_accuracy_1h_openml_alllosses_1h.tex <==
\begin{tabular}{lccccccc}
\toprule
  \textbf{Dataset} & \textbf{Auto-WEKA} & \textbf{auto-sklearn} &   \textbf{TPOT} & \textbf{H2O AutoML} & \textbf{GCP-Tables} & \textbf{AutoPilot} & \textbf{AutoGluon} \\
\midrule
        APSFailure &              0.007 &                 0.006 &           0.008 &               0.004 &               0.005 &              0.005 &     \textbf{0.004} \\
          Airlines &                 x  &                 0.331 &           0.356 &               0.378 &      \textbf{0.327} &              0.332 &              0.344 \\
            Albert &              0.379 &                 0.314 &           0.348 &               0.336 &               0.310 &              0.352 &     \textbf{0.307} \\
 Amazon\_employee\_a &              0.052 &        \textbf{0.050} &           0.052 &               0.050 &               0.054 &              0.054 &              0.051 \\
        Australian &     \textbf{0.130} &                    x  &  \textbf{0.130} &      \textbf{0.130} &                  x  &                 x  &     \textbf{0.130} \\
         Covertype &              0.357 &                 0.033 &           0.243 &               0.115 &               0.066 &                 x  &     \textbf{0.023} \\
            Dionis &     \textbf{0.114} &                    x  &           0.458 &                  x  &                  x  &                 x  &              0.163 \\
     Fashion-MNIST &              0.150 &                 0.120 &           0.232 &               0.106 &               0.100 &                 x  &     \textbf{0.097} \\
            Helena &              0.723 &                 0.670 &           0.676 &               0.628 &                  x  &              0.633 &     \textbf{0.628} \\
            Jannis &              0.355 &                    x  &           0.290 &               0.273 &               0.277 &              0.281 &     \textbf{0.271} \\
 KDDCup09\_appetenc &              0.019 &        \textbf{0.017} &  \textbf{0.017} &               0.024 &      \textbf{0.017} &     \textbf{0.017} &     \textbf{0.017} \\
         MiniBooNE &              0.095 &                 0.061 &           0.064 &               0.056 &               0.055 &              0.059 &     \textbf{0.053} \\
            Robert &                 x  &                 0.536 &              x  &      \textbf{0.502} &                  x  &                 x  &              0.507 \\
           Shuttle &       \textbf{0.0} &                 0.000 &           0.000 &               0.000 &                  x  &              0.000 &              0.000 \\
           Volkert &              0.379 &                 0.328 &           0.353 &               0.301 &               0.301 &              0.300 &     \textbf{0.265} \\
             adult &              0.144 &                 0.125 &           0.124 &               0.131 &               0.124 &              0.128 &     \textbf{0.123} \\
    bank-marketing &              0.092 &                 0.090 &           0.091 &               0.092 &               0.090 &              0.094 &     \textbf{0.089} \\
 blood-transfusion &               0.24 &                  0.24 &  \textbf{0.213} &               0.226 &                  x  &                 x  &               0.24 \\
               car &              0.208 &          \textbf{0.0} &    \textbf{0.0} &        \textbf{0.0} &        \textbf{0.0} &              0.005 &       \textbf{0.0} \\
         christine &              0.317 &                 0.265 &           0.267 &               0.263 &                  x  &              0.261 &     \textbf{0.249} \\
            cnae-9 &              0.148 &        \textbf{0.018} &  \textbf{0.018} &      \textbf{0.018} &                  x  &                 x  &              0.046 \\
         connect-4 &              0.292 &                 0.176 &           0.140 &               0.133 &      \textbf{0.119} &              0.135 &              0.128 \\
          credit-g &                0.2 &                    x  &   \textbf{0.19} &                0.22 &                  x  &                 x  &               0.21 \\
           dilbert &              0.027 &                 0.015 &           0.069 &               0.022 &                  x  &              0.021 &     \textbf{0.008} \\
            fabert &              0.396 &                 0.266 &           0.308 &               0.275 &               0.294 &              0.276 &     \textbf{0.265} \\
        guiellermo &                 x  &                 0.182 &             0.4 &               0.151 &                  x  &                 x  &     \textbf{0.149} \\
             higgs &              0.395 &                 0.268 &           0.272 &               0.277 &      \textbf{0.258} &              0.285 &              0.264 \\
           jasmine &              0.183 &                 0.170 &           0.187 &               0.183 &      \textbf{0.167} &              0.214 &              0.173 \\
 jungle\_chess\_2pcs &              0.254 &                 0.084 &           0.081 &               0.090 &      \textbf{0.001} &              0.045 &              0.009 \\
               kc1 &              0.142 &                 0.151 &           0.132 &               0.137 &               0.127 &                 x  &     \textbf{0.123} \\
          kr-vs-kp &              0.009 &        \textbf{0.003} &              x  &               0.006 &               0.006 &              0.006 &              0.006 \\
     mfeat-factors &     \textbf{0.015} &                  0.03 &           0.035 &               0.025 &                0.02 &              0.035 &               0.02 \\
             nomao &              0.022 &        \textbf{0.017} &           0.019 &               0.024 &               0.026 &              0.029 &              0.020 \\
       numerai28.6 &     \textbf{0.479} &                 0.488 &              x  &               0.494 &               0.481 &              0.488 &              0.489 \\
           phoneme &              0.077 &                 0.109 &           0.097 &               0.094 &               0.086 &              0.099 &     \textbf{0.075} \\
          riccardo &                 x  &                    x  &              x  &      \textbf{0.002} &                  x  &                 x  &     \textbf{0.002} \\
           segment &              0.012 &        \textbf{0.008} &           0.012 &      \textbf{0.008} &      \textbf{0.008} &              0.012 &     \textbf{0.008} \\
           sylvine &              0.076 &                 0.064 &           0.048 &               0.058 &               0.058 &              0.062 &     \textbf{0.042} \\
           vehicle &              0.141 &                 0.164 &  \textbf{0.129} &               0.141 &                  x  &                 x  &              0.152 \\
\bottomrule
\end{tabular}


==> tables/openml_alllosses_1h.tex <==
\begin{tabular}{lcccccc}
\toprule
  \textbf{Dataset} & \textbf{Auto-WEKA} & \textbf{auto-sklearn} &   \textbf{TPOT} & \textbf{H2O AutoML} & \textbf{GCP-Tables} & \textbf{AutoGluon} \\
\midrule
        APSFailure &              0.047 &                 0.006 &           0.011 &               0.008 &               0.005 &     \textbf{0.004} \\
          Airlines &                 x  &                 0.276 &           0.309 &      \textbf{0.267} &               0.271 &              0.291 \\
            Albert &              0.334 &                 0.250 &           0.294 &      \textbf{0.238} &               0.242 &              0.238 \\
 Amazon\_employee\_a &              0.180 &                 0.129 &  \textbf{0.118} &               0.120 &               0.129 &              0.118 \\
        Australian &     \textbf{0.045} &                    x  &           0.076 &               0.060 &                  x  &              0.050 \\
         Covertype &              1.070 &                 0.113 &           0.605 &               0.326 &               0.197 &     \textbf{0.058} \\
            Dionis &              1.277 &                    x  &           2.545 &                  x  &                  x  &     \textbf{0.964} \\
     Fashion-MNIST &              1.254 &                 0.389 &           0.792 &               0.300 &      \textbf{0.273} &              0.286 \\
            Helena &              9.134 &                 2.887 &           3.039 &               2.697 &                  x  &     \textbf{2.615} \\
            Jannis &              2.302 &                    x  &           0.736 &               0.676 &               0.676 &     \textbf{0.661} \\
 KDDCup09\_appetenc &              0.271 &                 0.167 &           0.179 &               0.182 &               0.154 &     \textbf{0.145} \\
         MiniBooNE &              0.084 &                 0.015 &           0.019 &               0.015 &               0.014 &     \textbf{0.014} \\
            Robert &                 x  &                 1.714 &              x  &      \textbf{1.563} &                  x  &              1.606 \\
           Shuttle &       \textbf{0.0} &                 0.000 &           0.000 &               0.001 &                  x  &              0.000 \\
           Volkert &              2.114 &                 0.919 &           1.005 &               0.837 &               0.839 &     \textbf{0.727} \\
             adult &              0.093 &                 0.069 &           0.071 &               0.069 &               0.068 &     \textbf{0.068} \\
    bank-marketing &              0.079 &                 0.061 &           0.063 &               0.061 &               0.061 &     \textbf{0.059} \\
 blood-transfusion &              0.236 &        \textbf{0.225} &           0.268 &               0.241 &                  x  &              0.231 \\
               car &              0.721 &                 0.005 &           0.002 &      \textbf{4e-05} &               0.000 &              0.000 \\
         christine &              0.231 &                 0.161 &           0.178 &               0.160 &                  x  &     \textbf{0.155} \\
            cnae-9 &              0.393 &                 0.087 &  \textbf{0.057} &               0.112 &                  x  &              0.145 \\
         connect-4 &              0.812 &                 0.470 &           0.358 &               0.350 &      \textbf{0.309} &              0.328 \\
          credit-g &              0.145 &                    x  &  \textbf{0.135} &               0.159 &                  x  &              0.154 \\
           dilbert &              0.515 &                 0.044 &           0.226 &               0.070 &                  x  &     \textbf{0.027} \\
            fabert &              2.514 &                 0.750 &           0.884 &               0.726 &               0.785 &     \textbf{0.652} \\
        guiellermo &                 x  &                 0.114 &           0.134 &               0.091 &                  x  &     \textbf{0.074} \\
             higgs &              0.355 &                 0.189 &           0.196 &               0.183 &      \textbf{0.179} &              0.182 \\
           jasmine &              0.133 &        \textbf{0.118} &           0.142 &               0.125 &               0.134 &              0.130 \\
 jungle\_chess\_2pcs &              0.618 &                 0.203 &           0.201 &               0.238 &      \textbf{0.007} &              0.025 \\
               kc1 &              0.141 &                 0.180 &           0.158 &               0.159 &               0.166 &     \textbf{0.135} \\
          kr-vs-kp &              0.000 &          \textbf{0.0} &              x  &               0.000 &               8e-05 &              4e-05 \\
     mfeat-factors &              0.122 &                 0.127 &           0.122 &               0.104 &               0.104 &     \textbf{0.074} \\
             nomao &              0.007 &        \textbf{0.001} &           0.002 &               0.003 &               0.004 &              0.002 \\
       numerai28.6 &              0.476 &                 0.476 &              x  &               0.477 &      \textbf{0.475} &              0.484 \\
           phoneme &              0.050 &                 0.037 &           0.036 &               0.034 &               0.033 &     \textbf{0.024} \\
          riccardo &                 x  &                    x  &              x  &      \textbf{0.000} &                  x  &     \textbf{0.000} \\
           segment &              0.239 &                 0.075 &           0.066 &               0.068 &               0.063 &     \textbf{0.047} \\
           sylvine &              0.021 &                 0.013 &  \textbf{0.008} &               0.015 &               0.020 &              0.013 \\
           vehicle &              0.817 &                 0.363 &           0.315 &      \textbf{0.303} &                  x  &              0.311 \\
\bottomrule
\end{tabular}

